Dual Supervision Framework for Relation Extraction with Distant Supervision and Human Annotation

Relation extraction (RE) has been extensively studied due to its importance in real-world applications such as knowledge base construction and question answering. Most of the existing works train the models on either distantly supervised data or human-annotated data. To take advantage of the high accuracy of human annotation and the cheap cost of distant supervision, we propose the dual supervision framework which effectively utilizes both types of data. However, simply combining the two types of data to train a RE model may decrease the prediction accuracy since distant supervision has labeling bias. We employ two separate prediction networks HA-Net and DS-Net to predict the labels by human annotation and distant supervision, respectively, to prevent the degradation of accuracy by the incorrect labeling of distant supervision. Furthermore, we propose an additional loss term called disagreement penalty to enable HA-Net to learn from distantly supervised labels. In addition, we exploit additional networks to adaptively assess the labeling bias by considering contextual information. Our performance study on sentence-level and document-level REs confirms the effectiveness of the dual supervision framework.

==> framework_old.tex <==

\section{Dual Supervision Framwork}
In this section, we propose our dual supervision framework to effectively use both human-labeled data and distant supervision data.
A straightforward method is to train a relation extraction model by using both types of data.
However, since distant supervision data is noisy and biased, the use of it can reduce extraction accuracy. 


To solve the problem, our framework builds two prediction networks instead of using a single prediction network for estimating the two heterogeneous labels.
One of the prediction networks estimate the human-annotated labels and it is used to extract relations from the test data.
The other prediction network estimates the labels obtained by distant supervision.
We call the first network \hanet and the second network \dsnet.



\subsection{Prediction networks}

Relation extraction models output the probability that $\triple{h}{r}{t}$ appears in document $d$.
We represent the output by $o_{h,t}(r) =$ $Pr(\triple{h}{r}{t} \text{ appears in } d)$.
Cross entropy loss is widely used as a loss function of existing relation extraction algorithms \cite{cai2016bidirectional, sorokin2017context, zeng2015distant, zeng2014relation}.
The cross entropy of an output is computed as
\begin{equation}
L_{h, t|d} = -\sum_{r \in R_{h,t|d}}{\log{o_{h,t}(r)}}-\sum_{r \notin R_{h,t|d}}{\log{(1-o_{h,t}(r))}}
\end{equation}
where $R_{h,t|d}=\{r|\triple{h}{r}{t} \text{ appears in } d\}$ is the set of relations between $h$ and $t$ that appear in document $d$.


With the two prediction networks, the proposed framework use the following loss function
\begin{equation}
L_{h, t|d} = L_{h,t|d}^{HA} + L_{h,t|d}^{DS} + \lambda \cdot L_{h,t|d}^{DS-HA}.
\end{equation}
As discussed in Section~\ref{sec:existing}, the loss function of existing methods measures the difference between estimated and true values for the data.
Similarly, the first term $L_{h,t|d}^{HA}$ and the second term $L_{h,t|d}^{DS}$ measure the discrepancy between the estimated values and the labels for human annotation data and distant supervision data, respectively.
We call $L_{h,t|d}^{DS-HA}$ the \emph{disagreement penalty}.
The disagreement penalty captures the distance between the estimations by \hanet and \dsnet.
$\lambda$ is a trade-off parameter that controls the relative importance of the prediction error and the disagreement penalty.
By using two separated prediction networks and introducing the disagreement penalty, \hanet can be learned from distant supervision labels while avoiding overfitting to distant supervision labels.



\subsection{The disagreement penalty}
As shown in Section~\ref{sec:intro}, distant supervision labels are biased and the bias size varies depending on the type of relation.
In addition, the size of the bias also can be different by many other features such as the types of head and tail entities, contents of the document or sentence.
Consequently, an effective disagreement penalty should consider the bias which depends on the context.
%with p-value 


Let $X$ be the random variable which denotes the distance between the estimates $o^{DS}_{h,t}(r)$ and $o^{HA}_{h,t}(r)$ (i.e., $X=o^{DS}_{h,t}(r)-o^{HA}_{h,t}(r)$).
We assume that the $X$ follows a normal distribution $\normal{\mu}{\sigma}$ where $\mu$ is the expected bias of the distant supervision label.
Since the bias varies depending on the context, we employ two additional networks, named \munet and \sigmanet, to predict the bias distribution.
\munet and \sigmanet estimate the mean $\mu$ and standard deviation $\sigma$ of the probability distribution of $X$.


The proposed disagreement penalty is defined as the negative log likelihood of the difference $o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r)$.
The log-likelihood of the difference is
\begin{equation}
\begin{aligned}
&-\log{p(o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r)| \mu, \sigma)} \\
&= -\frac{1}{2}\{\mu - (o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r))\}^2 - \log{\sigma} + \log{\pi}.
\end{aligned}
\end{equation}
Since $\log{\pi}$ is constant, we obtain the following disagreement penalty
\begin{equation}
 L_{h,t|d}^{DS-HA} = \frac{1}{2}\{\mu - (o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r))\}^2 + \log{\sigma}
\end{equation}
where $o^{HA}_{h,t}(r)$, $o^{DS}_{h,t}(r)$, $\mu$, and $\sigma$ are the outputs of \hanet, \dsnet, \munet, and \sigmanet modules, respectively.


\subsection{Training and testing}
We construct each training batch to have half of training instances with human-annotated labels and the other half of instances with distantly supervised labels.
The human-labeled documents do not necessarily have an overlap with the documents with distant supervision.
In our experiment, there was no overlap between the documents with human annotations and the documents with distant supervision.

For a training instance with human annotations the loss function is
%\begin{equation}
\begin{align}
	L_{h, t|d} &= L_{h,t|d}^{HA} + \lambda \cdot L_{h,t|d}^{DS-HA}\\
	&= -\sum_{r \in R_{h,t|d}^{HA}}{\log{o_{h,t}^{HA}(r)}}-\sum_{r \notin R_{h,t|d}^{HA}}{\log{(1-o_{h,t}^{HA}(r))}}\\
	&+ \lambda[\frac{1}{2}\{\mu_r - (o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r))\}^2 + \log{\sigma_r}]
\end{align}
%\end{equation}
where $R_{h,t|d}^{HA}$ is the set of typed relations that labeled by human annotation on the document $d$.
Similarly, the loss function for distant supervision is
\begin{align}
	L_{h, t|d} &= L_{h,t|d}^{DS} + \lambda \cdot L_{h,t|d}^{DS-HA}\\
	&= -\sum_{r \in R_{h,t|d}^{DS}}{\log{o_{h,t}^{DS}(r)}}-\sum_{r \notin R_{h,t|d}^{DS}}{\log{(1-o_{h,t}^{DS}(r))}}\\
	&+ \lambda[\frac{1}{2}\{\mu_r - (o^{DS}_{h,t}(r) - o^{HA}_{h,t}(r))\}^2 + \log{\sigma_r}]
\end{align}
%\end{equation}
where $R_{h,t|d}^{DS}$ is the set of typed relations that labeled by distant supervision on the document $d$.


In the test time, input document are given to the model and we take $o^{HA}_{h,t}(r)$ for $r \in R$ as the output of the model.
If $o^{HA}_{h,t}(r)$ is greater than a threshold, we regard that the model outputs the relational fact $\triple{h}{r}{t}$.
The threshold is tuned on development dataset.


==> intro_a.tex <==
\section{Introduction}
\label{sec:intro}
Relation extraction has been widely used in real-world applications such as knowledge base construction \cite{dong2014knowledge, KnowledgeFusion,JungKS19}, question answering \cite{xu2016question} and biomedical data mining \cite{ahmed2019bio}.
Given a text with a pair of entities, the goal of relation extraction is to discover the relationships between the entities in the text.
%Relation extraction has been extensively studied during the last decade due to its importance in real-world applications such as knowledge base construction \cite{dong2014knowledge, KnowledgeFusion,JungKS19} and question answering \cite{xu2016question}.
Neural relation extraction models usually represent the entities by vectors and feed the vectors to a classification module to find
the relations between them.
%Then, 

%Since the extracted relationships can be used to automatically build large-scale knowledge bases \cite{dong2014knowledge, KnowledgeFusion,JungKS19},
%it has been extensively studied during the last decade.


\begin{figure}[tb]
	%\adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}
	%\frame{
	%\begin{framed}\noindent
	\begin{flushleft}
		{\large \textsf{\bf Pacific Fair Shopping Centre}}
	\end{flushleft}
	\vspace{-0.04in}
	\tcbset{colback=brown!5!white}
	\begin{somebox}[left=3px, right=3px]
		Document \\
		 \entity{[Pacific Fair Shopping Centre:E1]} is a major shopping centre in Broadbeach Waters on the Gold Coast, \entity{[Queensland:E2]}, Australia. 
		 It was Queensland's largest regional shopping centre until 2006.
		 \entity{[Pacific Fair:E1]} was developed by \entity{[Hooker Retail Developments:E3]} and opened in \entity{[1977:E4]} on what was swampland with 96 specialty stores and two anchor tenants.
		 ...
		\tcblower
		Entities \\
		E1: \entity{Pacific Fair Shopping Centre}\\
		E2: \entity{Queensland}\\
		E3: \entity{Hooker Retail Development}\\
		E4: \entity{1977}\\
		...\\
		Relations \\
		R1: \triple{\text{\entity{E1}}} {\text{\relation{located\_in}}} {\text{\entity{E2}}}\\
		R2: \triple{\text{\entity{E1}}} {\text{\relation{developer}}} {\text{\entity{E3}}}\\
		R3: \triple{\text{\entity{E1}}} {\text{\relation{inception}}} {\text{\entity{E4}}}\\
		...
	\end{somebox}
	%\end{framed}
	%}
	\caption{An example of a document and relations  \label{fig:doc}}
\end{figure}



Existing works for relation extraction \cite{mintz2009distant,lin2016neural,zeng2014relation,zeng2015distant} mainly addressed the sentence-level relation extraction which finds the relations between entities in a sentence.
However, many relational facts are expressed across multiple sentences.
Recently, a large-scale document-level relation extraction (DocRED) dataset was published in \cite{yao2019docred} to accelerate the researches on document-level relation extraction.
% and some sentence-level algorithms \cite{cai2016bidirectional,zeng2014relation,sorokin2017context} were adopted for the document-level relation extraction in \cite{yao2019docred}.
%In \cite{wang2019fine}, a fine tuning model of BERT \cite{devlin2018bert} was proposed.
%One of the most distinctive characteristics of DocRED data is that 
%it contains
%the number of entity mentions tends to be larger than in sentence-level relation extraction.
%In the dataset, 
\red{Extending the relation extraction} from sentence-level to document-level enables finding the relational facts over multiple sentences\red{, however,} it brings a new challenge to researches on relation extraction.
An entity is usually mentioned once in a sentence.
Meanwhile, an entity tends to be mentioned in multiple sentences in a document.
In addition, each mention of an entity can be involved in a different relation.
%\memo{different relation for each occurence}
%However, in most cases, only one of the entity mentions of an entity involved in a relational fact.
%Thus, we may need a different representation of the same entity.
%///relation extraction - representation 
%While an entity is usually mentioned once in a sentence, it tends to be mentioned multiple times in a document.
Thus, for an entity appearing in a given document, depending on the other entity with which we need to find the relation, we may need a different representation of the same entity.
For example, consider \figurename~\ref{fig:doc} which shows a document and some relations in DocRED dataset.
Note that the entity `Pacific Fair Shopping Centre' is mentioned in the first and third sentences.
It is clear that we need to use the entity mention of `Pacific Fair Shopping Centre' in the first sentence to find the relation R1.
On the contrary, we need to use its entity mention in the third sentence to identify the relations with `Hooker Retail Developments' and `1977' (i.e., R2 and R3).
In this way, we need to use a different representation of an entity depending on the entity which we want to find the relation with.
However, existing works for document-level relation extraction \cite{yao2019docred, wang2019fine} simply represent an entity by the average of the representations of its entity mentions.
%To obtain a good representation of an entity, we propose an attention-based entity encoder which adaptively 
To overcome the drawback of utilizing the static representation for an entity, we propose an attention-based entity encoder to obtain an adaptive representation of an entity based on the other entity to be used to find the relations with.



To generate a dataset to train models for relation extraction, we can use either human annotation or distant supervision. %, we can use human annotations or distant supervision.
Human annotation provides high-quality labels to be used to train the relation extraction models.
However, since human labeling is expensive, it is difficult to build a large-scale dataset.
%the labels obtained by this method is usually not enough.
Thus, the distant supervision \cite{mintz2009distant}, which labels relations between entities using existing knowledge bases, is proposed to automatically produce a large-scale dataset.
Although we can obtain a large dataset by distant supervision,
distant supervision usually suffers from the wrong labeling problem.
To train models for document-level relation extraction, existing works \cite{wang2019fine, yao2019docred} utilized the datasets generated by either human annotation or distant supervision only.



To take advantage of the accuracy of human annotation and the large size of distant supervision, we propose to utilize a large distantly supervised (DS) data as well as a small amount of human-annotated (HA) data.
However, simply combining the two types of data to train a relation extraction model may decrease the accuracy since there exists a labeling bias in distant supervision.
To explain the bias,
%we first present a definition of inflation in distant supervision for a relation type $r$.
 let the inflation of a relation be the average frequency of the relation in DS data normalized by the average frequency in HA data.
 \red{If the inflation of a relation is 1, the relation appears equally frequently in the two types of data and the labels are not biased for the relation.}
%We can calculate the inflation by using the DS and HA data according to the following equation:
%\begin{equation*}
%Inflation(r) = \frac{\text{Avg. number of relation } r \text{ in DS data} }{\text{Avg. number of relation } r \text{ in HA data}}.
%\end{equation*}
In the document-level relation extraction dataset (DocRED) \cite{yao2019docred} has 96 relations and the inflations of the relations vary from 0.48 to 85.9.
In other words, distant supervision can generate tens of times more wrong labels than true labels for some relation types.
%We think this is a nature of distant supervision.
%The reason
%For example, many cities have their `sister cities'. 


For example, consider a part of DocRED dataset in \figurename~\ref{fig:bias_existing}.
For a document in the training data, distant supervision produces the label \triple{\ehead}{\relationt{sister\_city}}{\etail} when the two cities \head and \tail, which have `sister city' relationship in a knowledge base, appear in the document.
However, `sister city' relation rarely appears in human-annotated labels of DocRED because the relationship is not frequently expressed in the text data. 
Although we train a model with additional true labels obtained by human-annotation, this bias produced a significant number of false positives because the number of false labels is much larger than that of true labels.
For example, the state-of-the-art \cite{wang2019fine} outputs \triple{London}{\relationt{sister\_city}}{New York} for the text in the figure even though the `sister city' relationship is not represented in the text.  



%\memo{old}\\
%%Thus, 
%For example,......consider doc in fig 2.... many cities have their sister cities. 
%For a text (sentence or document) ..to generate?.. , distant supervision produces the label \triple{\ehead}{\relationt{sister\_city}}{\etail} when the two cities \head and \tail, which have `sister city' relationship in a knowledge base, appear in the text.
%However, `sister city' relation rarely appears in human-annotated labels of DocRED because the relationship is not frequently expressed in the text data. 
%%However, distant supervision produce many labels with `sister city' since many cities have their sister cities and they often appear in a same document
%This bias produces a significant number of false positives. 
%\figurename~\ref{fig:bias_existing} shows a part of DocRED dataset.
%As we discussed, training data obtained by distant supervision has a number of false labels for `sister city' relationships.
%Consequently, the state-of-the-art \cite{wang2019fine} outputs \triple{London}{\relationt{sister\_city}}{New York} for the text in the figure even though the `sister city' relationship is not represented in the text.
%\memo{----------}\\
%\memo{still has problem ds-ha}

\begin{figure}[tb]
	\includegraphics[width=3.33in]{example_existing}
	\caption{The problem of labeling bias in distantly supervised labels. \label{fig:bias_existing}}
\end{figure}



%\subsection{Existing Algorithms}
%\label{sec:existing}

\figurename~\ref{fig:existing_framework} shows an generic relation extraction model which consist of an encoding layer, an entity encoder and a prediction network.
The encoding layer encodes the given document to hidden representations. 
A previous work \cite{zeng2014relation} used distance between the two entities in addition to word embeddings.
Previous works \cite{cai2016bidirectional} and \cite{wang2019fine} exploited Bi-LSTM and BERT, respectively to effectively represent the context.
From the encoded text, entity encoder outputs the representations of head and tail entities.
To represent an entity, document-level relation extraction works \cite{yao2019docred,wang2019fine} averaged the representations of its entity mentions.
The prediction network outputs the probability that $\triple{h}{r}{t}$ appears in document $d$.
Multi-layer perceptron, bilinear layer\cite{wang2019fine} and convolutional neural networks \cite{zeng2014relation} have been used for the prediction network.

\begin{figure}[tb]
	\includegraphics[width=3.2in]{existing_framework_3steps}
	\caption{A general framework of exiting models for relation extraction \memo{Seoul}\label{fig:existing_framework}}
\end{figure}


To effectively use the two types of data, we propose the \red{dual supervision} framework.
An overview of the proposed model is shown in \figurename~\ref{fig:proposed_model_overall}.
Following the state-of-the-art \cite{wang2019fine}, we use BERT \cite{devlin2018bert} to encode the input text.
Unlike the previous work, we employ two prediction networks \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
This allows the difference in the estimations for human annotations and distant supervision.
Consequently, it prevents the accuracy decrease by the wrong labels from distant supervision.
In addition, we use two additional networks \munet and \sigmanet for modeling the disagreement between the outputs of \hanet and \dsnet.
%Our framework exploits two prediction modules named \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
%By 
%In addition, we observed that the distribution of the inflation follows a log-normal distribution.
%#In addition, we model the disagreement of the outputs of \hanet and \dsnet.
%In addition, we impose a regularization
% model the disagreement of the outputs of \hanet and \dsnet by a log-normal distribution.
Our experimental results confirm that our dual supervision framework significantly improved the accuracy compared to simply using the two types of data to train a model with a single prediction module.




\begin{figure}[tb]
	\includegraphics[width=3.25in]{proposed_model_overall_3steps}
	\caption{The overall architecture of the proposed model\label{fig:proposed_model_overall}}
\end{figure}


%As reported in a series of previous works \cite{lin2016neural}, distant supervision usually  from wrong labeling problem.






The contributions of our paper are summarized as follows:
\begin{itemize}
	\item We identified the bias of labels obtained by distant supervision. In addition, we analyzed the distribution of the bias by using a real-life dataset.
	\item Based on the analysis of the labeling bias of distant supervision, we proposed a framework to effectively utilize distant supervision data and human annotation data.
	\item We devise a cross attention entity encoder to find relations between many pairs of entity mentions. 
	\item With an extensive experiment on a real-life datatset, we show that our proposed algorithm outperforms the existing algorithms.
		We also empirically demonstrated the effectiveness of the dual supervision framework and the cross attention entity encoder.
\end{itemize}






==> intro_shim.tex <==
\section{Introduction}
\label{sec:intro}
Relation extraction has been widely used in real-world applications such as knowledge base construction \cite{dong2014knowledge, KnowledgeFusion,JungKS19}, question answering \cite{xu2016question} and biomedical data mining \cite{ahmed2019bio}.
Given a text with a pair of entities, the goal of relation extraction is to discover all relationships between the entities expressed in the text.
%Relation extraction has been extensively studied during the last decade due to its importance in real-world applications such as knowledge base construction \cite{dong2014knowledge, KnowledgeFusion,JungKS19} and question answering \cite{xu2016question}.
Early studies for relation extraction \cite{mintz2009distant,riedel2010modeling, hoffmann2011knowledge} utilize hand-crafted features obtained by existing NLP tools such as dependency parser and POS tagger.
However, since the relation extraction models take the input features from NLP tools, the errors \red{brought by NLP} tools \red{are propagated} to the models \red{used in the relation extraction methods}.
Toc\red{overcome such problems}, recent works \cite{lin2016neural,zeng2014relation,zeng2015distant,sorokin2017context, wang2019fine} \red{apply} deep neural networks in relation extraction instead of using handcrafted features.
Deep learning models for relation extraction \red{typically} represent the entities by vectors and feed \red{them} to a classification module to find the relations between \red{the entities}.

%Then, 

%Since the extracted relationships can be used to automatically build large-scale knowledge bases \cite{dong2014knowledge, KnowledgeFusion,JungKS19},
%it has been extensively studied during the last decade.


\begin{figure}[tb]
	%\adjustbox{margin=1em,width=\textwidth,set height=4cm,set depth=4cm,frame,center}
	%\frame{
	%\begin{framed}\noindent
	\begin{flushleft}
		{\large \textsf{\bf Pacific Fair Shopping Centre}}
	\end{flushleft}
	\vspace{-0.04in}
	\tcbset{colback=brown!5!white}
	\begin{somebox}[left=3px, right=3px]
		Document \\
		 \entity{[Pacific Fair Shopping Centre:E1]} is a major shopping centre in Broadbeach Waters on the Gold Coast, \entity{[Queensland:E2]}, Australia. 
		 It was Queensland's largest regional shopping centre until 2006.
		 \entity{[Pacific Fair:E1]} was developed by \entity{[Hooker Retail Developments:E3]} and opened in \entity{[1977:E4]} on what was swampland with 96 specialty stores and two anchor tenants.
		 ...
		\tcblower
		Entities \\
		E1: \entity{Pacific Fair Shopping Centre}\\
		E2: \entity{Queensland}\\
		E3: \entity{Hooker Retail Development}\\
		E4: \entity{1977}\\
		...\\
		Relations \\
		R1: \triple{\text{\entity{E1}}} {\text{\relation{located\_in}}} {\text{\entity{E2}}}\\
		R2: \triple{\text{\entity{E1}}} {\text{\relation{developer}}} {\text{\entity{E3}}}\\
		R3: \triple{\text{\entity{E1}}} {\text{\relation{inception}}} {\text{\entity{E4}}}\\
		...
	\end{somebox}
	%\end{framed}
	%}
	\caption{An example of a document and relations  \label{fig:doc}}
\end{figure}



Existing works for relation extraction \cite{mintz2009distant,lin2016neural,zeng2014relation,zeng2015distant} mainly \red{focus on} the \red{sentence-level extraction} which finds the relations between entities in a sentence.
However, many relational facts are expressed across multiple sentences.
Recently, a large-scale document-level relation extraction (DocRED) dataset was published in \cite{yao2019docred} to accelerate research on document-level relation extraction.
\red{It is reported in \cite{yao2019docred} that} 46.4\% of the relation instances are \red{associated} with multiple sentences \red{in the dataset} and 40.7\% of the relational \red{facts} cannot be found by the \red{sentence-level extraction}.
% and some sentence-level algorithms \cite{cai2016bidirectional,zeng2014relation,sorokin2017context} were adopted for the document-level relation extraction in \cite{yao2019docred}.
%In \cite{wang2019fine}, a fine tuning model of BERT \cite{devlin2018bert} was proposed.
%One of the most distinctive characteristics of DocRED data is that 
%it contains
%the number of entity mentions tends to be larger than in sentence-level relation extraction.
%In the dataset, 
Extending the relation extraction from sentence-level to document-level enables us to find the relational facts over multiple sentences.
However, it brings a new \red{challenge} to the problem of relation extraction.
%An entity is usually mentioned once in sentence-level while it tends to be mentioned multiple times in document-level.
An entity \red{generally appears} once in a sentence.
Meanwhile, an entity tends to be mentioned in multiple sentences in a document.
In addition, each mention of an entity can be involved in a different relation.
%\memo{different relation for each occurence}
%However, in most cases, only one of the entity mentions of an entity involved in a relational fact.
%Thus, we may need a different representation of the same entity.
%///relation extraction - representation 
%While an entity is usually mentioned once in a sentence, it tends to be mentioned multiple times in a document.
Thus, for an entity \red{occurring} in a given document, depending on the other entity with which we need to find the relation, we may need different representations of the same entity.


\red{Consider an exampl with a document and some relations in DocRED dataset shown in \figurename~\ref{fig:doc}}.
Note that the entity `Pacific Fair Shopping Centre' \red{appears} in the first and third sentences.
It is clear that we need to use the entity mention of `Pacific Fair Shopping Centre' in the first sentence to find the relation with `Queensland' (i.e. R1).
On the contrary, we need to use its entity mention in the third sentence to identify the relations with `Hooker Retail Developments' and `1977' (i.e., R2 and R3).
In other words, we should dynamically represent an entity depending on the entity which we want to find the relation with.
However, existing works for document-level relation extraction \cite{yao2019docred, wang2019fine} simply represent an entity by the average of the representations of its entity mentions.
%To obtain a good representation of an entity, we propose an attention-based entity encoder which adaptively 
To overcome the drawback of utilizing the static representation for an entity, we propose an attention-based entity encoder to obtain an adaptive representation of an entity based on the other entity to be used to find the relations with.



To generate a dataset to train models for relation extraction, we can use either human annotation or distant supervision. %, we can use human annotations or distant supervision.
Human annotation provides high-quality labels to be used to train the relation extraction models.
However, since human labeling is expensive, it is difficult to produce a large-scale dataset.
%the labels obtained by this method is usually not enough.
Thus, the distant supervision \cite{mintz2009distant}, which labels \red{the} relations between entities using existing knowledge bases, is proposed to automatically produce a large-scale dataset.
Although we can obtain a large dataset by distant supervision,
it \red{typically} suffers from the wrong labeling problem.
Existing works \cite{wang2019fine, yao2019docred} utilize the datasets generated by either human annotation or distant supervision only although each of the two labeling methods has a clear weakness.



To take advantage of the accuracy of human annotation and the large size of distant supervision, we propose to utilize a large distantly supervised (DS) data as well as a small amount of human-annotated (HA) data.
However, simply combining the two types of data to train a relation extraction model may decrease the prediction accuracy since there exists a \emph{labeling bias} in distant supervision.
To explain the bias,
%we first present a definition of inflation in distant supervision for a relation type $r$.
 let the inflation of a relation be the frequency of the relation in DS data divided by the frequency in HA data.
 When a relation label occurs with the same frequency in the two types of data, the inflation of the relation becomes 1 and we say that the labels of the relation are not biased.
%We can calculate the inflation by using the DS and HA data according to the following equation:
%\begin{equation*}
%Inflation(r) = \frac{\text{Avg. number of relation } r \text{ in DS data} }{\text{Avg. number of relation } r \text{ in HA data}}.
%\end{equation*}
The document-level relation extraction dataset (DocRED) \cite{yao2019docred} has 96 relation types and the inflations of the relation types vary from 0.48 to 85.9.
In other words, distant supervision can generate tens of times more \red{incorrect} labels than true labels for some relation types.
%We think this is a nature of distant supervision.
%The reason
%For example, many cities have their `sister cities'. 


\red{Consider} some documents of DocRED dataset in \figurename~\ref{fig:bias_existing}.
For a document in the training data, distant supervision produces the label \triple{\ehead}{\relationt{sister\_city}}{\etail}\red{,} when the two cities \head and \tail, which have `sister city' relationship in a knowledge base, appear in the document.
However, `sister city' relation rarely appears in human-annotated labels of DocRED \red{dataset} because the relationship is not frequently expressed in the text data. 
Although we train a model with additional true labels obtained by human-annotation, this bias produces a significant number of false positives \red{since} the number of false labels is much larger than that of true labels.
For example, the state-of-the-art \cite{wang2019fine} for document-level relation extraction produces \triple{London}{\relationt{sister\_city}}{New York} for the test document in \figurename~\ref{fig:bias_existing}, even though the `sister city' relationship is not represented in the text.  



%\memo{old}\\
%%Thus, 
%For example,......consider doc in fig 2.... many cities have their sister cities. 
%For a text (sentence or document) ..to generate?.. , distant supervision produces the label \triple{\ehead}{\relationt{sister\_city}}{\etail} when the two cities \head and \tail, which have `sister city' relationship in a knowledge base, appear in the text.
%However, `sister city' relation rarely appears in human-annotated labels of DocRED because the relationship is not frequently expressed in the text data. 
%%However, distant supervision produce many labels with `sister city' since many cities have their sister cities and they often appear in a same document
%This bias produces a significant number of false positives. 
%\figurename~\ref{fig:bias_existing} shows a part of DocRED dataset.
%As we discussed, training data obtained by distant supervision has a number of false labels for `sister city' relationships.
%Consequently, the state-of-the-art \cite{wang2019fine} outputs \triple{London}{\relationt{sister\_city}}{New York} for the text in the figure even though the `sister city' relationship is not represented in the text.
%\memo{----------}\\
%\memo{still has problem ds-ha}

\begin{figure}[tb]
	\includegraphics[width=3.33in]{example_existing}
	\caption{An example of wrong extraction result caused by the labeling bias of distant supervision. The state-of-the-art \cite{wang2019fine} produced many similar false relations although we used both human annotated-labels and distant supervision for training the model. \label{fig:bias_existing}}
\end{figure}



%\subsection{Existing Algorithms}
%\label{sec:existing}

%\figurename~\ref{fig:existing_framework} shows \underline{a} generic relation extraction model 

%A generic model for relation extractions consists of a text encoder, an entity encoder and a prediction network.
Existing neural relation extraction models consist of a text encoder, an entity encoder and a prediction network.
The text encoder converts a given document to hidden representations. 
%The existing work in \cite{zeng2014relation} uses the distance between the two entities in addition to word embeddings, while the methods in \cite{cai2016bidirectional} and \cite{wang2019fine} exploit Bi-LSTM and BERT, respectively to effectively consider the context too.
From the encoded text, the entity encoder generates the representations of the head entity \head and tail entity \tail.
%To represent an entity, the existing works \cite{yao2019docred,wang2019fine} for document-level relation extraction utilized the average of the representation vectors of its entity mentions.
The prediction network outputs the probability that $\triple{\ehead}{r}{\etail}$ appears in the document for every relation $r$.
%Multi-layer perceptrons, bilinear layers\cite{wang2019fine} and convolutional neural networks \cite{zeng2014relation} have been used for the prediction network.

To effectively utilize the two types of data generated by human annotations and distant supervision, we propose the dual supervision framework.
As the state-of-the-art \cite{wang2019fine} does, we use BERT \cite{devlin2018bert} to encode the input text. For the prediction layer, 
unlike the previous works that utilize a single prediction network, we employ two prediction networks \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
\memo{How about attention?}
This allows the difference in the estimations for human annotations and distant supervision.
Consequently, it prevents the accuracy degradation by the incorrect labels produced by distant supervision.
In addition, we apply two additional networks \munet and \sigmanet to model the disagreement between the outputs of \hanet and \dsnet. 
Our experimental results confirm that our dual supervision framework significantly improved the accuracy compared to simply using the two types of data to train a model with a single prediction network.






%Our framework exploits two prediction modules named \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
%By 
%In addition, we observed that the distribution of the inflation follows a log-normal distribution.
%#In addition, we model the disagreement of the outputs of \hanet and \dsnet.
%In addition, we impose a regularization
% model the disagreement of the outputs of \hanet and \dsnet by a log-normal distribution.




%As reported in a series of previous works \cite{lin2016neural}, distant supervision usually  from wrong labeling problem.






The contributions of our paper are summarized as follows:
\begin{itemize}
	\item We identified the bias of labels obtained by distant supervision. In addition, we analyzed the distribution of the bias by using a real-life dataset.
	\item Based on the analysis of the labeling bias of distant supervision, we proposed a framework to effectively utilize distant supervision data and human annotation data.
	\item We devise a cross attention entity encoder to find relations between many pairs of entity mentions. 
	\item With an extensive experiment on a real-life datatset, we show that our proposed algorithm outperforms the existing algorithms.
		We also empirically demonstrated the effectiveness of the dual supervision framework and the cross attention entity encoder.
\end{itemize}






==> proposed.tex <==
%\section{The Proposed Model}
%In this section, we present a model for relation extraction which utilizes the dual supervision framework proposed in the previous section. 

\begin{wrapfigure}{R}{0.45\textwidth}
	%\begin{center}
	\includegraphics[width=0.43\textwidth]{entity_encoder}
	%\end{center}
	\caption{Cross-attention entity encoder \label{fig:entity_encoder}}
\end{wrapfigure}
%\begin{figure}[tb]
%	\centering
%	\hspace{0.2in}
%	\includegraphics[width=2.2in]{entity_encoder}
%	\vspace{-0.05in}
%	\caption{Cross-attention entity encoder \label{fig:entity_encoder}}
%\end{figure}

\section{Cross-Attention Entity Encoder for Document-level RE}
The structure of our cross-attention entity encoder is shown in \figurename~\ref{fig:entity_encoder}.
Our entity encoder takes the word vectors $\hat{\vect{x}}_i$s produced by the text encoder as input.
It obtains the intermediate representations $\vect{h}_0$ and $\vect{t}_0$ of the head and tail entities.
Note that the entity encoders in \cite{yao2019docred,wang2019fine} output these vectors.
Instead, we generate the head entity vector $\vect{h}$ and tail entity vector $\vect{t}$ based on the intermediate representation by using two attention networks.
We call both networks the cross-attention entity encoder.



Let $\hat{\vect{x}}_i$ denote the word vector of the $i$-th word in a given document produced by the text encoder.
For each entity mention $m_k$ ranging from the $b$-th word to the $e$-th word in the document, let us denote its representation $\vect{m}_k$ by $\frac{1}{e-b+1} \sum_{i=b}^{e}{\hat{\vect{x}}_i}$. Then, the intermediate representation of an entity (i.e., $\vect{h}_0$ and $\vect{t}_0$) is defined as the average of the representations of its entity mentions.
Specifically, we have
\begin{equation*}
\vect{h}_0 = \frac{1}{|M_h|} \sum_{k \in M_{h}}{\vect{m}_k},~~\vect{t}_0 = \frac{1}{|M_t|} \sum_{k \in M_{t}}{\vect{m}_k}
\end{equation*}
where $M_{h}$ and $M_{t}$ are the mentions of the head and tail entities, respectively.
Note that the intermediate representation of the head entity $h_0$ is independently computed from the tail entity.
Thus, we always get the same intermediate representation of the head entity regardless of the tail entity although the text encoder has enough model capacity.
Since previous works \cite{yao2019docred,wang2019fine} use this representation in the prediction network, they use the same representation for an entity in a document.
However,each mention of an entity can be involved in a different relationship with a different entity.
Thus, it is desirable to adaptively generate the head entity vector based on the tail entity, and vice versa.





Motivated by the observation, we apply the attention mechanism \cite{bahdanau2015neural} to encode an entity by considering the other entity.
By using the intermediate representation of the tail entity $\vect{t}_0$, we first compute a $|W_h|$-dimensional attention vector, denoted by $\vect{\alpha}^h$, over the words in the head entity mentions where $W_h$ is the set of word indexes of the head entity mentions.
The attention vector is computed by
\begin{equation*}
\vect{\alpha}^h = Softmax(\vect{v}_h^\top tanh(\vect{U}_h \vect{x}_i + \vect{V}_h\vect{t}_0 + \vect{b}_h))
\end{equation*}
where $\vect{v}_h$, $\vect{U}_h$, $\vect{V}_h$ and $\vect{b}_h$ are the learnable parameters of the attention network.
Then, we take the weighted sum of the word embeddings over the words in the head entity mentions to compute the head entity vector $\vect{h}$.
That is, we have
\begin{equation*}
\vect{h} = \sum_{i \in W_h}{\alpha_i^h \hat{\vect{x}}_i}.
\end{equation*}



The tail entity vector  $\vect{t}$ and its  attention vector $\vect{\alpha}^t$ are similarly computed as
\begin{equation*}
\vect{\alpha}^t = Softmax(\vect{v}_t^\top tanh(\vect{U}_t \vect{x}_i + \vect{V}_t\vect{h}_0 + \vect{b}_t)), \vect{t} = \sum_{i \in W_t}{\alpha^t_i \hat{\vect{x}}_i}.
\end{equation*}


%Similarly, the tail entity vector $\vect{t}$ is obtained by another attention layer.
%The attention vector $\vect{\alpha}^t$ over the words in the tail entity mentions is computed as
%\begin{equation*}
%\vect{\alpha}^t = Softmax(\vect{v}_t^\top tanh(\vect{U}_t \vect{x}_i + \vect{V}_t\vect{h}_0 + \vect{b}_t))
%\end{equation*}
%where $\vect{v}_t$, $\vect{U}_t$, $\vect{V}_t$ and $\vect{b}_t$ are the learnable parameters of the attention network.
%The tail entity vector $\vect{t}$ is computed by
%\begin{equation*}
%\vect{t} = \sum_{i \in W_t}{\alpha^t_i \hat{\vect{x}}_i}.
%\end{equation*}











\iffalse
\subsection{A common structure of the modules}

\begin{figure}[tb]
	\includegraphics[width=2.2in]{common_module}
	\caption{A common structure of the modules of our proposed model \label{fig:common_module}}
\end{figure}
\fi




==> proposed_shim.tex <==
\section{The Proposed Model}
In this section, we present a model for relation extraction which utilizes the dual supervision framework proposed in the previous section. 



\subsection{\red{The Architecture}}
\begin{figure}[tb]
	\includegraphics[width=3.25in]{proposed_model_overall_3steps}
	\caption{The overall architecture of the proposed model\label{fig:proposed_model_overall}}
\end{figure}

The structure of our model \red{is summarized in \figurename~\ref{fig:proposed_model_overall}. It is made up of} a text encoder, a cross-attention entity encoder and an output layer with 4 sub-networks.

\red{Following the existing work \cite{wang2019fine}}, we use BERT \cite{devlin2018bert} to encode the document.
BERT is a pre-trained language model which is flexible to be fine-tuned for many NLP tasks.
Thus, it enables us to use simple structures for the entity encoder and the output layer.
Let $\vect{x}_i$ denote the embedding of \red{the} $i$-th word in a given document obtained from the BERT model.
For each word in \red{the} entity mentions of \red{the} head and tail \red{entities}, we use a linear layer to \red{calculate} an embedding to \red{be given} as an input for the entity encoder \red{by the following expression}
\begin{equation*}
	\hat{\vect{x}}_i = \vect{W}\vect{x}_i +\vect{b}
\end{equation*}
where $\vect{W}$ and $\vect{b}$ are \red{the} trainable parameters.

As \red{we} discussed in Section~\ref{sec:intro}, an entity can be involved in a different relationship depending \red{on} the other entity which we want to find the relation with.
To obtain an adaptive representation of an entity that features the other entity, we propose a novel entity encoder, \red{called the} cross-attention entity encoder, by using the attention mechanism \red{to be presented later} in Section~\ref{sec:entity_encoder}.

%\subsection{Overall structure}
%An overview of the proposed model is shown in \figurename~\ref{fig:proposed_model_overall}.
%Following the state-of-the-art \cite{wang2019fine}, we use BERT \cite{devlin2018bert} to encode the input text.
%Unlike the previous work, we employ two prediction networks \hanet and \dsnet to allow the difference in.
%In addition, we use two additional networks \munet and \sigmanet for modeling  the disagreement penalty.
%An overview of the proposed model is shown in \figurename~\ref{fig:proposed_model_overall}.
%Following the state-of-the-art \cite{wang2019fine}, we use BERT \cite{devlin2018bert} to encode the input text.


Unlike the previous work, we employ two prediction networks \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
This allows the difference in the estimations \red{of the labels} for human annotations and distant supervision.
Consequently, it prevents the accuracy decrease by the \red{incorrect (undesirable)} labels from distant supervision.
In addition, we use two additional networks \munet and \sigmanet for modeling the disagreement between the outputs of \hanet and \dsnet.
We will present the detailed structures of the networks in Section~\ref{sec:output_layer}.






%\subsection{Text encoder}
%Following the state-of-the-art \cite{wang2019fine} of document-level relation extraction, we use BERT \cite{devlin2018bert} to encode the document.
%BERT is a pre-trained language model which is flexible to be fine-tuned for many NLP tasks.
%Thus, it enables us to use simple structures for the entity encoder and the output layer.
%Let $\vect{x}_i$ denote the embedding of $i$-th word in a given document obtained from the BERT model.
%For each word in entity mentions of head and tail entity, we use a linear layer to compute an embedding to used as an input for the entity encoder:
%\begin{equation*}
%	\hat{\vect{x}}_i = \vect{W}\vect{x}_i +\vect{b}
%\end{equation*}
%where $\vect{W}$ and $\vect{b}$ are trainable parameters.


%\underline{ (This section is too small! Did other papers do the same thing?)}



\subsection{Cross-attention entity encoder}
\label{sec:entity_encoder}
The structure of our cross-attention entity encoder is \red{shown} in \figurename~\ref{fig:entity_encoder}.
Our entity encoder takes the word embeddings $\hat{\vect{x}}_i$s \red{produced by} the text encoder as input.
\red{It} first obtains the intermediate representations $\vect{h}_0$ and $\vect{t}_0$ of the head and tail entities, \red{as it was  doen  in} \cite{yao2019docred, wang2019fine} for document-level relation extraction.
	Then, we next \red{generte} the head entity vector $\vect{h}$ and tail entity vector $\vect{t}$ by using two attention networks. \red{We call both networks the} cross-attention entity encoder. \red{(Wuhwan, I cannot find "build a vector" in google!)}
	
	
	
	Let $\vect{x}_i$ denote the embedding of \red{the} $i$-th word in a given document \red{produced by} the text encoder.
	For each entity mention $m_k$ ranging from the $b$-th word to the $e$-th word \red{in the document}, \red{let us denote} its representation $\vect{m}_k$ by $\frac{1}{e-b+1} \sum_{i=b}^{e}{\hat{\vect{x}}_i}$. Then, the intermediate representation of an entity \red{(i.e.,  $\vect{h}_0$ and $\vect{t}_0$)} is given by the average of the representations of \red{its entity} mentions. \red{ In other words, we have}
	\begin{equation}
	\vect{h}_0 = \frac{1}{|M_h|} \sum_{k \in M_{h}}{\vect{m}_k},~~~~~~~\vect{t}_0 = \frac{1}{|M_t|} \sum_{k \in M_{t}}{\vect{m}_k}
	\end{equation}
	where $M_{h}$ and $M_{t}$ are the mentions of the head and tail entities, respectively.
	Note that the intermediate representation of the head entity $h_0$ is independently computed from the tail entity.
	Thus, we always get the same \red{interediate} representation of the head entity regardless of the tail entity although the text encoder has enough model capacity.
	However, as we \red{pointed out previously with} the example in \figurename~\ref{fig:doc}, each mention of an entity can be involved in a different relationship with a different entity.
	Thus, it is desirable to adaptively denote the \red{interediate} representation of the head entity based on the tail entity, and vice versa.
	
	
	\begin{figure}[tb]
		\centering
		\hspace{0.2in}
		\includegraphics[width=2.2in]{entity_encoder}
		\caption{Attention based entity encoder\label{fig:entity_encoder}}
	\end{figure}
	
	Motivated by the observation, we apply the attention mechanism \cite{bahdanau2015neural} to encode an entity by considering the other entity.
	By using the intermediate representation of the tail entity $\vect{t}_0$, we first compute a $|W_h|$-dimensional attention vector, denoted by $\vect{\alpha}^h$, over the words in the head entity mentions by
	\begin{equation}
	\vect{\alpha}^h = Softmax(\vect{v}_h^\intercal tanh(\vect{U}_h \vect{x}_i + \vect{V}_h\vect{t}_0 + \vect{b}_h))
	\end{equation}
	where $W_h$ is the set of word indexes of the head entity mentions. \red{Wuhan, there is no $W_h$. What is $\vect{U}_h$ and $vect{U}_h$ and $\vect{b}_h$? Define them)} 
	Then, the head entity vector $\vect{h}$ is computed as the weighted sum of the word embeddings over the words in head entity mentions. \red{That is, we have}
	\begin{equation}
	\vect{h} = \sum_{i \in W_h}{\alpha_i^h \hat{\vect{x}}_i}.
	\end{equation}
	
	Similarly, the tail entity vector $\vect{t}$ is \red{first} obtained by another attention layer.
	The $|W_t|$-dimensional attention vector $\vect{\alpha}^t$ over the words in the tail entity mentions is \red{next calculated} as
\begin{equation*}
\vect{\alpha}^t = Softmax(\vect{v}_t^\intercal tanh(\vect{U}_t \vect{x}_i + \vect{V}_t\vect{h}_0 + \vect{b}_t))
\end{equation*}
where \red{We have the same problem of not defining the symbols in the above.)} $W_t$ is the set of word indexes of the tail entity mentions.
\red{Finally,} the tail entity vector $\vect{t}$ is computed by
\begin{equation*}
\vect{t} = \sum_{i \in W_h}{\alpha^t_i \hat{\vect{x}}_i}.
\end{equation*}


\subsection{Output layer}
\label{sec:output_layer}
The output layer takes the head entity vector $\vect{h}$ and tail entity vector $\vect{t}$ from the attention-based entity encoder as input.
It consists of two prediction networks \hanet and \dsnet as well as two parameter networks \munet and \sigmanet.
The prediction networks \hanet and \dsnet output the $|R|$-dimensional vectors $\vect{o}^{HA}_{h,t}=[p^{HA}_1,...$ $,p^{HA}_{|R|})]$ and $\vect{o}^{DS}_{h,t} = [p^{DS}_1, ...,p^{DS}_{|R|}]$ , respectively.
The parameter networks \munet and \sigmanet output $\vect{\mu}=[\mu_1,...,\mu_{|R|}]$ and $\vect{\sigma}=[\sigma_1,...,\sigma_{|R|}]$, respectively which are
the parameters of the log-normal distributions to represent the disagreement penalty.


%Recall that the inflation follows a log-normal distribution: $\frac{o^{DS}_{h,t}(r)}{o^{HA}_{h,t}(r)} \sim LogNormal(\mu_r, \sigma_r)$.

\minisection{Prediction networks}
We used the same structure of the prediction network in the previous works \cite{yao2019docred, wang2019fine} for our prediction networks.
We first concatenate the input with distance embedding:
\begin{equation}
\hat{\vect{h}}= [\vect{h};\vect{E}(d_{h,t})], \hat{\vect{t}}= [\vect{t};\vect{E}(d_{t,h})]\\
\end{equation}
where $[\cdot;\cdot]$ denotes concatenation, $d_{h,t}$ and $d_{t,h}$ are the relative distances of the first occurrence of the two entities, and  $\vect{E}(d)$ is the embedding of relative distance $d$.
Then, we apply a Bi-Linear layer and a sigmoid function to find the relations between the head and tail entities.
Specifically, we obtain the output of \hanet as 
\begin{equation}
\vect{o}^{HA}_{h,t} = sigmoid(BiLinear^{HA}(\hat{\vect{h}}, \hat{\vect{t}}))
\end{equation}
where $BiLinear^{HA}$ is a BiLinear layer for \hanet and a Bi-linear layer is defined as follows:
\memo{eq}
%\begin{equation*}
%BiLinear({\vect{x}, \vect{y})) = \vect{x}^\intercal.
%\end{equation*}
Similarly, the output of \dsnet is defined as 
\begin{equation}
\vect{o}^{DS}_{h,t} = sigmoid(BiLinear^{DS}(\hat{\vect{h}}, \hat{\vect{t}})).
\end{equation}
%\begin{equation}
%P(r|\vect{h}, \vect{t}) = sigmoid(\hat{\vect{h}} \vect{W}_r^{HA} \hat{\vect{t}} + b_r^{HA})\\
%\end{equation}
%where $\vect{W}_r^{HA}$, $b_r^{HA}$ are learnable parameters for relation $r$.
%
%Similarly,
%\begin{equation}
%	\begin{aligned}
%	\hat{\vect{h}}= [\vect{h};\vect{E}(d_{h,t})], \hat{\vect{t}}= [\vect{t};\vect{E}(d_{t,h})]\\% \[ \vect{h}  Ed_{h,t} \] \hat{\vect{t}}= \[\vect{t}; E(d_{t,h})\]\\
%	P(r|\vect{h}, \vect{t}) = sigmoid(\hat{\vect{h}} \vect{W}_r^{HA} \hat{\vect{t}} + b_r^{HA})
%	\end{aligned}
%\end{equation}
%where $[\cdot;\cdot]$ denotes concatenation, $d_{h,t}$ and $d_{t,h}$ are the relative distances of the first occurrence of the two entities, $\vect{E}(d)$ is the embedding of the relative distance $d$, and $\vect{W}_r^{HA}$, $b_r^{HA}$ are learnable parameters for relation $r$.
% which output  $\vect{o}^{HA}$, $\vect{o}^{DS}$, $\vect{\mu}$ and $\vect{\sigma}$, respectively.
%Each of the output modules consists of a Bi-Linear layer and an activation function.
%Since $\vect{o}^{HA}$ and $\vect{o}^{DS}$ represent the probabilities of 
%, we use the sigmoid as the activation function of \hanet and \dsnet.
%

\minisection{Parameter networks}
The structures of \munet and \sigmanet are also similar except the activation functions.
For a log-normal distribution $Lognormal(\mu, \sigma)$, the parameter $\mu$ can be positive or negative and $\sigma$ is a positive value.
Thus, we use a hyperbolic tangent function and a softplus function \cite{dugas2001incorporating} as the activation functions of \munet and \sigmanet, respectively.
Formally, the parameter vector $\vect{\mu}$ is computed as
\begin{equation}
\vect{\mu} = tanh(BiLinear^{\mu}(\hat{\vect{h}}, \hat{\vect{t}})).
\end{equation}
and the parameter vector $\vect{\sigma}$ is computed as
\begin{equation}
\vect{\sigma} = softplus(BiLinear^{\sigma}(\hat{\vect{h}}, \hat{\vect{t}})) + \varepsilon
\end{equation}
where $softplus(x) = \log{(1+e^x)}$ and $\varepsilon$ is a sanity bound to prevent the variance goes to zero.
We set the sanity bound $\varepsilon$ to 0.001.









\iffalse
\subsection{A common structure of the modules}

\begin{figure}[tb]
	\includegraphics[width=2.2in]{common_module}
	\caption{A common structure of the modules of our proposed model \label{fig:common_module}}
\end{figure}



\begin{table}
	\caption{Activation functions of the modules}
	\label{tab:activation}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l l}
				\toprule
				{\bf Module} & {\bf Activation function}\\
				\midrule
				\hanet & Sigmoid\\
				\dsnet & Sigmoid\\
				\munet & Leaky ReLU\\
				\sigmanet & Softplus\\
				\bottomrule
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}
\fi



==> proposed_shim2.tex <==
\section{The Proposed Model}
In this section, we present a model for relation extraction which utilizes the dual supervision framework proposed in the previous section. 



\subsection{\red{The Architecture}}
\begin{figure}[tb]
	\includegraphics[width=3.25in]{proposed_model_overall_3steps}
	\caption{The overall architecture of the proposed model\label{fig:proposed_model_overall}}
\end{figure}

The structure of our model \red{is summarized in \figurename~\ref{fig:proposed_model_overall}. It is made up of} a text encoder, a cross-attention entity encoder and an output layer with 4 sub-networks.

\red{Following the existing work \cite{wang2019fine}}, we use BERT \cite{devlin2018bert} to encode the document.
BERT is a pre-trained language model which is flexible to be fine-tuned for many NLP tasks.
Thus, it enables us to use simple structures for the entity encoder and the output layer.
Let $\vect{x}_i$ denote the embedding of \red{the} $i$-th word in a given document obtained from the BERT model.
For each word in \red{the} entity mentions of \red{the} head and tail \red{entities}, we use a linear layer to \red{calculate} an embedding to \red{be given} as an input for the entity encoder \red{by the following expression}
\begin{equation*}
	\hat{\vect{x}}_i = \vect{W}\vect{x}_i +\vect{b}
\end{equation*}
where $\vect{W}$ and $\vect{b}$ are \red{the} trainable parameters.

As \red{we} discussed in Section~\ref{sec:intro}, an entity can be involved in a different relationship depending \red{on} the other entity which we want to find the relation with.
To obtain an adaptive representation of an entity that features the other entity, we propose a novel entity encoder, \red{called the} cross-attention entity encoder, by using the attention mechanism \red{to be presented later} in Section~\ref{sec:entity_encoder}.

%\subsection{Overall structure}
%An overview of the proposed model is shown in \figurename~\ref{fig:proposed_model_overall}.
%Following the state-of-the-art \cite{wang2019fine}, we use BERT \cite{devlin2018bert} to encode the input text.
%Unlike the previous work, we employ two prediction networks \hanet and \dsnet to allow the difference in.
%In addition, we use two additional networks \munet and \sigmanet for modeling  the disagreement penalty.
%An overview of the proposed model is shown in \figurename~\ref{fig:proposed_model_overall}.
%Following the state-of-the-art \cite{wang2019fine}, we use BERT \cite{devlin2018bert} to encode the input text.


Unlike the previous work, we employ two prediction networks \hanet and \dsnet to estimate the labels by human annotation and distant supervision, respectively.
This allows the difference in the estimations \red{of the labels} for human annotations and distant supervision.
Consequently, it prevents the accuracy decrease by the \red{incorrect (undesirable)} labels from distant supervision.
In addition, we use two additional networks \munet and \sigmanet for modeling the disagreement between the outputs of \hanet and \dsnet.
We will present the detailed structures of the networks in Section~\ref{sec:output_layer}.






%\subsection{Text encoder}
%Following the state-of-the-art \cite{wang2019fine} of document-level relation extraction, we use BERT \cite{devlin2018bert} to encode the document.
%BERT is a pre-trained language model which is flexible to be fine-tuned for many NLP tasks.
%Thus, it enables us to use simple structures for the entity encoder and the output layer.
%Let $\vect{x}_i$ denote the embedding of $i$-th word in a given document obtained from the BERT model.
%For each word in entity mentions of head and tail entity, we use a linear layer to compute an embedding to used as an input for the entity encoder:
%\begin{equation*}
%	\hat{\vect{x}}_i = \vect{W}\vect{x}_i +\vect{b}
%\end{equation*}
%where $\vect{W}$ and $\vect{b}$ are trainable parameters.


%\underline{ (This section is too small! Did other papers do the same thing?)}



\subsection{Cross-attention entity encoder}
\label{sec:entity_encoder}
The structure of our cross-attention entity encoder is \red{shown} in \figurename~\ref{fig:entity_encoder}.
Our entity encoder takes the word embeddings $\hat{\vect{x}}_i$s \red{produced by} the text encoder as input.
\red{It} first obtains the intermediate representations $\vect{h}_0$ and $\vect{t}_0$ of the head and tail entities, \red{as it was  doen  in} \cite{yao2019docred, wang2019fine} for document-level relation extraction.
	Then, we next \red{generte} the head entity vector $\vect{h}$ and tail entity vector $\vect{t}$ by using two attention networks. \red{We call both networks the} cross-attention entity encoder. \red{(Wuhwan, I cannot find "build a vector" in google!)}
	
	
	
	Let $\vect{x}_i$ denote the embedding of \red{the} $i$-th word in a given document \red{produced by} the text encoder.
	For each entity mention $m_k$ ranging from the $b$-th word to the $e$-th word \red{in the document}, \red{let us denote} its representation $\vect{m}_k$ by $\frac{1}{e-b+1} \sum_{i=b}^{e}{\hat{\vect{x}}_i}$. Then, the intermediate representation of an entity \red{(i.e.,  $\vect{h}_0$ and $\vect{t}_0$)} is given by the average of the representations of \red{its entity} mentions. \red{ In other words, we have}
	\begin{equation}
	\vect{h}_0 = \frac{1}{|M_h|} \sum_{k \in M_{h}}{\vect{m}_k},~~~~~~~\vect{t}_0 = \frac{1}{|M_t|} \sum_{k \in M_{t}}{\vect{m}_k}
	\end{equation}
	where $M_{h}$ and $M_{t}$ are the mentions of the head and tail entities, respectively.
	Note that the intermediate representation of the head entity $h_0$ is independently computed from the tail entity.
	Thus, we always get the same \red{interediate} representation of the head entity regardless of the tail entity although the text encoder has enough model capacity.
	However, as we \red{pointed out previously with} the example in \figurename~\ref{fig:doc}, each mention of an entity can be involved in a different relationship with a different entity.
	Thus, it is desirable to adaptively denote the \red{interediate} representation of the head entity based on the tail entity, and vice versa.
	
	
	\begin{figure}[tb]
		\centering
		\hspace{0.2in}
		\includegraphics[width=2.2in]{entity_encoder}
		\caption{Attention based entity encoder\label{fig:entity_encoder}}
	\end{figure}
	
	Motivated by the observation, we apply the attention mechanism \cite{bahdanau2015neural} to encode an entity by considering the other entity.
	By using the intermediate representation of the tail entity $\vect{t}_0$, we first compute a $|W_h|$-dimensional attention vector, denoted by $\vect{\alpha}^h$, over the words in the head entity mentions where $W_h$ is the set of word indexes of the head entity mentions.
	The attention vector is computed by
	\begin{equation}
	\vect{\alpha}^h = Softmax(\vect{v}_h^\intercal tanh(\vect{U}_h \vect{x}_i + \vect{V}_h\vect{t}_0 + \vect{b}_h))
	\end{equation}
	where  $\vect{v}_h$, $\vect{U}_h$, $\vect{U}_h$ and $\vect{b}_h$ are the learnable parameters of the attention network.
	Then, the head entity vector $\vect{h}$ is computed as the weighted sum of the word embeddings over the words in head entity mentions. \red{That is, we have}
	\begin{equation}
	\vect{h} = \sum_{i \in W_h}{\alpha_i^h \hat{\vect{x}}_i}.
	\end{equation}
	
	Similarly, the tail entity vector $\vect{t}$ is \red{first} obtained by another attention layer.
	The $|W_t|$-dimensional attention vector $\vect{\alpha}^t$ over the words in the tail entity mentions is \red{next calculated} as
\begin{equation*}
\vect{\alpha}^t = Softmax(\vect{v}_t^\intercal tanh(\vect{U}_t \vect{x}_i + \vect{V}_t\vect{h}_0 + \vect{b}_t))
\end{equation*}
where \red{We have the same problem of not defining the symbols in the above.)} $W_t$ is the set of word indexes of the tail entity mentions.
\red{Finally,} the tail entity vector $\vect{t}$ is computed by
\begin{equation*}
\vect{t} = \sum_{i \in W_h}{\alpha^t_i \hat{\vect{x}}_i}.
\end{equation*}


\subsection{Output layer}
\label{sec:output_layer}
The output layer takes \red{as input the head and tain entity vectors $\vect{h}$ and  $\vect{t}$ from the attention-based entity encoder}.
It consists of two prediction networks \hanet and \dsnet as well as two parameter networks \munet and \sigmanet.
The prediction networks \hanet and \dsnet output the $|R|$-dimensional vectors $\vect{o}^{HA}_{h,t}=[p^{HA}_1,...$ $,p^{HA}_{|R|})]$ and $\vect{o}^{DS}_{h,t} = [p^{DS}_1, ...,p^{DS}_{|R|}]$ , respectively, \red{where $R$ is a set of possible relation types}.
The parameter networks \munet and \sigmanet  \red{ also} output \red{the vectors}  $\vect{\mu}=[\mu_1,...,\mu_{|R|}]$ and $\vect{\sigma}=[\sigma_1,...,\sigma_{|R|}]$, respectively\red{,} which are
the parameters of the log-normal distributions to represent the disagreement penalty.


%Recall that the inflation follows a log-normal distribution: $\frac{o^{DS}_{h,t}(r)}{o^{HA}_{h,t}(r)} \sim LogNormal(\mu_r, \sigma_r)$.

\minisection{Prediction networks}
We \red{use} the same structure of the prediction network \red{in \cite{yao2019docred, wang2019fine}} for our prediction networks.
We first concatenate the input with distance embedding:
\begin{equation}
\hat{\vect{h}}= [\vect{h};\vect{E}(d_{h,t})], \hat{\vect{t}}= [\vect{t};\vect{E}(d_{t,h})]\\
\end{equation}
where $[\cdot;\cdot]$ denotes \red{ the concatenation of two vectors}, $d_{h,t}$ and $d_{t,h}$ are the relative distances \red{between} the first occurrence of the two entities, and  $\vect{E}(d)$ is the embedding of relative distance $d$. \red{what is the relative distance? Define it)}
Then, we apply a Bi-Linear layer and a sigmoid function to find the relations between the head and tail entities.
Specifically, we \red{compute} the output of \hanet as 
\begin{equation}
\vect{o}^{HA}_{h,t} = sigmoid(BiLinear^{HA}(\hat{\vect{h}}, \hat{\vect{t}}))
\end{equation}
where $BiLinear^{HA}$ is a BiLinear layer for \hanet and a Bi-linear layer is defined as follows:
\memo{eq}
%\begin{equation*}
%BiLinear({\vect{x}, \vect{y})) = \vect{x}^\intercal.
%\end{equation*}
Similarly, the output of \dsnet is \red{calculated} as 
\begin{equation}
\vect{o}^{DS}_{h,t} = sigmoid(BiLinear^{DS}(\hat{\vect{h}}, \hat{\vect{t}}))
\end{equation}
\red{where $BiLinear^{DS}$ is a BiLinear layer for \hanet.}
%\begin{equation}
%P(r|\vect{h}, \vect{t}) = sigmoid(\hat{\vect{h}} \vect{W}_r^{HA} \hat{\vect{t}} + b_r^{HA})\\
%\end{equation}
%where $\vect{W}_r^{HA}$, $b_r^{HA}$ are learnable parameters for relation $r$.
%
%Similarly,
%\begin{equation}
%	\begin{aligned}
%	\hat{\vect{h}}= [\vect{h};\vect{E}(d_{h,t})], \hat{\vect{t}}= [\vect{t};\vect{E}(d_{t,h})]\\% \[ \vect{h}  Ed_{h,t} \] \hat{\vect{t}}= \[\vect{t}; E(d_{t,h})\]\\
%	P(r|\vect{h}, \vect{t}) = sigmoid(\hat{\vect{h}} \vect{W}_r^{HA} \hat{\vect{t}} + b_r^{HA})
%	\end{aligned}
%\end{equation}
%where $[\cdot;\cdot]$ denotes concatenation, $d_{h,t}$ and $d_{t,h}$ are the relative distances of the first occurrence of the two entities, $\vect{E}(d)$ is the embedding of the relative distance $d$, and $\vect{W}_r^{HA}$, $b_r^{HA}$ are learnable parameters for relation $r$.
% which output  $\vect{o}^{HA}$, $\vect{o}^{DS}$, $\vect{\mu}$ and $\vect{\sigma}$, respectively.
%Each of the output modules consists of a Bi-Linear layer and an activation function.
%Since $\vect{o}^{HA}$ and $\vect{o}^{DS}$ represent the probabilities of 
%, we use the sigmoid as the activation function of \hanet and \dsnet.
%

\minisection{Parameter networks}
The structures of \munet and \sigmanet are also similar except the activation functions.
For a log-normal distribution $Lognormal(\mu, \sigma)$, the parameter $\mu$ can be positive or negative\red{, but $\sigma$ is always a positive value}.
Thus, we use a hyperbolic tangent function and a softplus function \cite{dugas2001incorporating} as the activation functions of \munet and \sigmanet, respectively.
\red{More specifically}, the parameter vector $\vect{\mu}$ is computed as
\begin{equation}
\vect{\mu} = tanh(BiLinear^{\mu}(\hat{\vect{h}}, \hat{\vect{t}}))
\end{equation}
and the parameter vector $\vect{\sigma}$ is calculated as
\begin{equation}
\vect{\sigma} = softplus(BiLinear^{\sigma}(\hat{\vect{h}}, \hat{\vect{t}})) + \varepsilon
\end{equation}
where $softplus(x) = \log{(1+e^x)}$ and $\varepsilon$ is a sanity bound to prevent the variance goes to zero.
We set the sanity bound $\varepsilon$ to 0.001.









\iffalse
\subsection{A common structure of the modules}

\begin{figure}[tb]
	\includegraphics[width=2.2in]{common_module}
	\caption{A common structure of the modules of our proposed model \label{fig:common_module}}
\end{figure}



\begin{table}
	\caption{Activation functions of the modules}
	\label{tab:activation}
	\begin{minipage}{\columnwidth}
		\begin{center}
			\begin{tabular}{l l}
				\toprule
				{\bf Module} & {\bf Activation function}\\
				\midrule
				\hanet & Sigmoid\\
				\dsnet & Sigmoid\\
				\munet & Leaky ReLU\\
				\sigmanet & Softplus\\
				\bottomrule
			\end{tabular}
		\end{center}
	\end{minipage}
\end{table}
\fi


